Muse: Text-To-Image Generation via Masked Generative Transformers

We present Muse, a text-to-image Transformer model that achieves state-of-the-art image generation performance while being significantly more efficient than diffusion or autoregressive models. Muse is trained on a masked modeling task in discrete token space: given the text embedding extracted from a pre-trained large language model (LLM), Muse is trained to predict randomly masked image tokens. Compared to pixel-space diffusion models, such as Imagen and DALL-E 2, Muse is significantly more efficient due to the use of discrete tokens and requiring fewer sampling iterations; compared to autoregressive models, such as Parti, Muse is more efficient due to the use of parallel decoding. The use of a pre-trained LLM enables fine-grained language understanding, translating to high-fidelity image generation and the understanding of visual concepts such as objects, their spatial relationships, pose, cardinality etc. Our 900M parameter model achieves a new SOTA on CC3M, with an FID score of 6.06. The Muse 3B parameter model achieves an FID of 7.88 on zero-shot COCO evaluation, along with a CLIP score of 0.32. Muse also directly enables a number of image editing applications without the need to fine-tune or invert the model: inpainting, outpainting, and mask-free editing. More results are available at https://muse-model.github.io

==> figs/model_sizes.tex <==

\begin{table}[t]

\vspace{5pt}
\label{tab:cc3m}
\begin{center}{
  \begin{tabular}{r r r }
\toprule
 \bfseries{Model Params} &
  \bfseries{Training Loss} 
 \bfseries{MS-COCO Zero-shot FID} & 
\\ 
\toprule
\name-0.6B & 6.8 & 0.25 \\
\name-1.2B & 6.06 & 0.26 \\
\name-3B & 6.06 & 0.26 \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Effects of scaling \name models. We show training losses, zero-shot FID scores (left), and the CLIP-FID curves on
MS-COCO (right).
\label{tbl:model_size}
\end{table}

==> vqgan_finetune_config.tex <==
%auto-ignore
\begin{table}[ht!]
\tablestyle{6pt}{1.02}
\scriptsize
\begin{tabular}{y{107}|y{150}}
Configuration & Value \\
\shline

Perceptual loss weight & 0.005 \\
Adversarial loss weight & 0.1 \\
Codebook size & 8192 \\
Optimizer & Adam \citep{KingmaB14} \\
Discriminator learning rate & 1e-4 \\
Generator learning rate & 1e-4 \\
Weight decay  & 1e-4 \\
Optimizer momentum & $\beta_1{=}0.9, \beta_2{=}0.99$ \\
Batch size & 256 \\
Learning rate schedule & cosine decay \citep{Loshchilov2017SGDRSG} \\
Warmup steps \citep{Goyal2017AccurateLM} & 10000 \\
Training steps & 1M

\end{tabular}
\vspace{-.5em}
\caption{Configuration and training hyperparameters for VQGAN Finetuning.}
\label{tab:vqgan} \vspace{-.5em}
\end{table}
